Exploring QUIC Dynamics: A Large-Scale Dataset for Encrypted Traffic Analysis

The increasing adoption of the QUIC transport protocol has transformed encrypted web traffic, necessitating new methodologies for network analysis. However, existing datasets lack the scope, metadata, and decryption capabilities required for robust benchmarking in encrypted traffic research. We introduce VisQUIC, a large-scale dataset of 100,000 labeled QUIC traces from over 44,000 websites, collected over four months. Unlike prior datasets, VisQUIC provides SSL keys for controlled decryption, supports multiple QUIC implementations (Chromium QUIC, Facebooks mvfst, Cloudflares quiche), and introduces a novel image-based representation that enables machine learning-driven encrypted traffic analysis. The dataset includes standardized benchmarking tools, ensuring reproducibility. To demonstrate VisQUICs utility, we present a benchmarking task for estimating HTTP/3 responses in encrypted QUIC traffic, achieving 97% accuracy using only observable packet features. By publicly releasing VisQUIC, we provide an open foundation for advancing encrypted traffic analysis, QUIC security research, and network monitoring.

==> sections/3-methods.tex <==
\subsection{Trace collection and image generation}
The process starts with HTTP/3~\cite{rfc9114} GET requests that are generated to various web servers that support HTTP/3, each hosting multiple websites. The websites were selected from the Tranco list~\cite{tranco}, which provides a ranking of the most visited domains while being resistant to manipulation. From this list, we identified websites hosted on servers supporting HTTP/3 through active probing, resulting in our final selection of web servers shown in Table~\ref{tab:combined-table}.

Data collection was performed from three distinct vantage points to ensure diverse network conditions: (1) a university network with a 1Gbps connection, (2) a cloud-hosted virtual machine in AWS's Europe region with 10Gbps connectivity, and (3) a residential network connection in the United States with 100Mbps bandwidth. This diversity in collection points helps capture how QUIC behaves under different network conditions and geographical distances from servers.

Requests are issued for up to 26,000 different websites per web server, with the actual number varying based on server capacity and availability. To ensure consistent experimental conditions and minimize noise in the collected data, we use Headless Chrome~\cite{headless} version 118.0.5993.70 in incognito mode with the application cache disabled. This methodological choice deliberately creates a controlled environment where each connection maintains identical baseline conditions, eliminating variations from cookies, cached content, and session states that could introduce unwanted artifacts into the traffic patterns. The apparent imbalance in website numbers across servers (e.g., Cloudflare hosting 26,738 sites versus Wiggle's 4) reflects the real-world distribution of HTTP/3 adoption, where certain providers like Cloudflare have extensively deployed QUIC while others are in earlier stages of adoption.

The generated network traffic traces are captured using Tshark~\cite{merino2013instant} in packet capture (PCAP) format. These traces include only QUIC packets and cover the duration of the website request. For each PCAP file the corresponding SSL keys are stored to be used later to decrypt the traffic. The SSL keys are also provided in the dataset's materials. Once we retain the time-series captured traces, the image datasets generation process can start for these traces. By Converting network traffic data---such as packet arrival times, packet sizes, packet density, and packet directions---into images the data is transformed into a format that is more compatible with DL models.

The use of images enhances pattern recognition abilities~\cite{farrukh2023senet, golubev2022image, shapira2019flowpic,tobiyama2016malware,velan2015survey}. Images enable the capture of complex interactions between features like packet sizes and arrival times within a two-dimensional space (server-to-client and client-to-server). This spatial representation allows DL models to identify intricate patterns that might be missed by traditional statistical or time-series analysis methods. For instance, correlations between packet bursts and response delays may become more discernible when visualized as variations in pixel intensity within an image. 
%%%%%% - end of new text.

Figure~\ref{fig:image-const} shows an example of the construction steps for an image with a window length of $0.3$ seconds from a trace. During step (a), some of the trace statistics are collected: the time when the observer sees this packet, the packet's length, and the packet's direction. For a 0.3-second window, each bin contains $9.375$ milliseconds. Step (b) shows histograms with $M=32$ time bins for the considered window. The upper one is for the packets sent by the server and the lower one is for packets sent by the client. The horizontal axis represents the time bins and the vertical axis represents the number of packets received during each bin. For example, in the $8$-th time bin (boxed in orange), the server sent $10$ packets and the client sent $19$ packets. Step (c) shows the image constructed for the considered example. The image represents the packet length statistics and the number of packets. 

Figure~\ref{fig:extended-miniflowpic} shows an example of the constructed image. The image is constructed on an $M \times N$ equispaced grid. The horizontal dimension represents different time window locations, while the vertical dimension represents different packet lengths. Thus, each packet is binned into one of the $M \times N$ bins according to its length and time. In the resulting image, the pixel at location $(i, j)$ represents the normalized number of packets whose length falls within the $j$-th bin received during the temporal span of the $i$-th time bin. The pixel's RGB values represent the normalized number of packets (i.e., density) sent from the server to the client (red) and from the client to the server (green). The blue channel is unused. The time interval spanned by the $i$-th bin is $[i \Delta t, (i+1) \Delta t )$, where $\Delta t = T / M$ and $T$ denotes the window length. In our experiments, we used $T=0.1$ and $T=0.3$ seconds. To be counted in length bin $j$, the length of a packet should be in the range of $[j \Delta l, (j+1) \Delta l]$ with $\Delta l = L / N$ and $L=1,500$ bytes denoting the maximum transmission unit (MTU). Histogram counts are normalized per channel window-wise using min-max normalization~\cite{patro2015normalization}, $x_{\mathrm{nrm}} = (x-x_\mathrm{min})/(x_\mathrm{max}-x_\mathrm{min})$, where $x$ and $x_{\mathrm{nrm}}$ are the original and normalized packet counts, respectively, and $x_\mathrm{min}$ and $x_\mathrm{max}$ are the minimum and maximum values of the packet count for the specific direction in the considered window, respectively. The normalized value is multiplied by 255 to fit an 8-bit image format. If there is no traffic for a specific window, all pixels will contain the value zero. Note that the shortest QUIC packet is longer than what is represented by the first length bin. Therefore, the first row of the image grid consistently exhibits pixels with a value of zero.

Figure~\ref{fig:extended-miniflowpic} shows different densities for each channel. For example, during time bin $i=7$, different shades of green are displayed. This indicates that the client sent packets of five different lengths, which fall into bins $j=2, 6, 12, 27$, and $28$. The five pixels are purely green, indicating that all the packets observed during bin $i=7$ were sent by the client. The brightness of a pixel increases as its value approaches 255. Pixel $(7,12)$ is the brightest across the whole window in the green channel and it represents $8$ packets. This means that the largest number of packets sent by the client during the window is observed during time bin $i=7$, when their length fell in bin $j=12$. The other green pixels represent between 2 to 5 packets that are sent by the client. At time bin $i=23$, the server sent packets of four different lengths, which are classified, based on their length, into bins $j=7, 10, 15$, and $17$. The four pixels are purely red, indicating that during time bin $i=23$, only packets sent by the server are observed. Pixel $(23, 10)$, representing $18$ packets, is the brightest within the red channel across the entire window. The rest of the red pixels represent between 3 and 15 packets sent by the server. Pixel $(9, 26)$ is a combination of green and red, indicating that during time bin $i=9$, packets from both the client and the server are observed and their length puts them into bin $j=26$.
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{figforpaper/image-temlate.pdf}
    \caption{An image template, representing QUIC connection activity. Pixel positions represent histogram bins (horizontal and vertical axes corresponding to time and packet length, respectively). The values of the red and green channels represent normalized, per-window, histogram counts of the response and request packets, respectively.}
    \label{fig:extended-miniflowpic}
\end{wrapfigure}

The image construction is an extension of the technique proposed by FlowPic~\cite{shapira2019flowpic}, which transforms network flows into images. For each flow, FlowPic creates an image from the packet lengths and the packet observed time. The goal of FlowPic is to construct a greyscale image using a flow-based two-dimensional histogram. FlowPic’s single-channel approach, while providing a general traffic overview, is insufficient for more nuanced analysis, particularly in the context of QUIC. In QUIC, distinguishing between client-to-server and server-to-client traffic is critical due to the multiplexed nature of HTTP/3 requests and responses. Furthermore, QUIC’s inherent complexity—stemming from stream multiplexing and independent packet handling—necessitates a more detailed examination of traffic directions. For those reasons we build upon the FlowPic technique and enhance it. We introduce a density factor for the packets' count in a given window and a configurable number of bins; in addition, we also separate channels, one for each direction. The result is an RGB image. Figure \ref{fig:different-responses} shows different images using a different number of pixels. Using a higher number of pixels leads to more detailed representation of the captured information. For example, a yellow pixel in Figure \ref{fig:different-responses}(\subref{fig:16}) which contains packets in both directions (a combination of the red and green channels), is split into more pixels as the resolution level is increased (Figures \ref{fig:different-responses}(\subref{fig:32}) and \ref{fig:different-responses}(\subref{fig:64})), resulting in solely red or green pixels.

\subsection{Dataset creation}
For the creation of the image dataset in our example use case, several key parameters were defined: the sliding window length, normalization method, and pixel resolution. Specifically, we generated two image datasets with the following configurations: (1) two different sliding window lengths of $T=0.1$ and $T=0.3$ seconds; (2) images sized at $M=N=32$, selected as a balance between resolution and computational cost. Using finer bins increased both the training and inference time with minimal accuracy improvement, while coarser bins negatively impacted model performance; and (3) normalization applied per window rather than per trace. For the baseline example, we utilized a 90\% overlap between consecutive windows during training, with no overlap during evaluation. The resulting labeled image dataset originates from over 100,000 traces collected from more than 44,000 websites, generating over seven million images.

\textbf{Labeling the images:} Each image in this dataset is labeled with the number of observed HTTP/3 responses; namely, the number of responses that have started to arrive within every time window. To this end, the SSL keys are used to decrypt the packets in a trace and reveal the packets' payloads. The HTTP/3 frames then are analyzed and HTTP/3 HEADERS frames are identified. Similarly, instead of labeling the images with the number of responses, the number of requests can be used as a label instead.

\subsection{Training and test sets}
The dataset can be split into two different settings: when the web servers are known to the observer and when they are not. In the former case, training and evaluation phases are done exclusively on the QUIC traces pertaining to the web servers assumed at inference time, using a $80:20$ ratio, ensuring out-of-training-sample evaluation. In the latter case, a leave-$x$-servers-out evaluation can be performed. For the provided use-case we show for the first setting results.
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.7\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figforpaper/01-dataset-distribution-v5.pdf}
        \vspace{-2mm}
        \caption{$T=0.1$ window dataset}
        \label{fig:01-window-length}
    \end{subfigure}%
    \vspace{5mm}
    \begin{subfigure}{0.7\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figforpaper/03-dataset-distribution-v5.pdf}
        \vspace{-2mm}
        \caption{$T=0.3$ window dataset}
        \label{fig:03-window-length}
    \end{subfigure}%
    \caption{Response distribution for training and evaluation datasets with two sliding window lengths ($T=0.1$ and $T=0.3$ seconds).}
    \label{fig:response-distribution}
\end{figure}

Figure \ref{fig:response-distribution} shows the images distribution for the created datasets. Both datasets are significantly skewed. As the figure demonstrates, images whose class values are $10$ or more are infrequent in both datasets. In the $T=0.1$-second window dataset, labels $0,1$ and $2$ make up roughly $75\%$ of the data, with the higher classes being represented in smaller proportions. Conversely, in the $T=0.3$-second window dataset, there is a more even distribution, with labels $0,1$ and $2$ comprising only about $47\%$ of the total dataset.   

\subsection{Discussion:}
\textbf{Selecting the window length: }The window length determines the temporal span each image represents, which directly impacts the data granularity. Shorter window lengths, such as $0.1$ seconds, capture fine-grained temporal details of the network traffic, allowing for detailed analysis of short-term interactions between the client and server. This high granularity level is very useful for identifying subtle variations and transient behaviors in the traffic. Using shorter windows, however,  also means generating a larger number of images per trace, leading to increased computational requirements. Conversely, longer window lengths, such as $0.3$ seconds or more, offer a more aggregated view of the traffic, encapsulating longer sequences of packet interactions within each image. This approach reduces the number of images generated, thereby decreasing computational demands. Longer windows are beneficial for capturing broader trends and interactions over extended periods, which can be advantageous for understanding overall traffic patterns and behaviors. The trade-off between short and long window lengths is a potential loss of fine-grained details, which might be critical for certain types of predictions. The choice of window length, therefore, should balance the need for temporal resolution with the practical considerations of computational efficiency.

\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-16.png}
        \caption{$16 \times 16$}
        \label{fig:16}
    \end{subfigure}%
    \hspace{1mm}
    \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-32.png}
        \caption{$32 \times 32$}
        \label{fig:32}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}{0.23\textwidth}
        \centering
    \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-64.png}
        \caption{$64 \times 64$}
        \label{fig:64}
    \end{subfigure}%
    \hspace{1mm}
    % \\[4mm] % Adjust the length as needed
    \begin{subfigure}{0.30\textwidth}
        \centering
    \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-128.png}
        \caption{$128 \times 128$}
        \label{fig:128}
    \end{subfigure}%
    \hspace{1mm}
    \begin{subfigure}{0.30\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-256.png}
        \caption{$256 \times 256$}
        \label{fig:256}
    \end{subfigure}
    \caption{Five examples of the image representation of QUIC flows using $T=0.1$-second windows and different pixels level.}
    \label{fig:different-responses}
\end{figure}

\textbf{Choosing the Resolution Level:} Selecting the image size involves balancing resolution, computational efficiency, and the ability of ML models to extract meaningful features. Common image sizes, such as $32 \times 32$, $64 \times 64$, and $256 \times 256$ pixels, each offer specific trade-offs. A $32 \times 32$ image is highly efficient in terms of computation, storage, and processing speed, making it ideal for real-time analysis or situations with limited resources. However, the lower resolution may fail to capture complex network behaviors, which could limit model accuracy. Increasing the resolution to $64 \times 64$ pixels strikes a better balance between detail and computational efficiency. This resolution captures more intricate traffic features—such as packet inter-arrival times, traffic pattern variations, burstiness, and transmission rate changes—while keeping the processing overhead manageable. On the higher end, $256 \times 256$ images provide the finest level of detail, making them suitable for tasks requiring high precision and sensitivity to subtle variations in traffic. However, this higher resolution comes at the cost of increased computational demands, longer processing times, and greater storage requirements, which may be impractical for real-time or large-scale applications. Additionally, the interpretation of each pixel’s resolution varies with window length, as each \say{bin} represents a portion of that window. Thus, the choice of resolution must be carefully aligned with the specific analysis goals and computational constraints.

\textbf{Normalizing per window versus per trace:} Normalizing the number of packet counts per window involves scaling the packet counts within each temporal window independently. This ensures that each window's data are scaled relative to its own range, which is beneficial for highlighting short-term variations and dynamics in network traffic. By normalizing per window, the resulting images maintain a consistent scale regardless of the overall trace length or variability across different windows or web servers. This approach helps mitigate the impact of outliers within individual windows, enabling the model to detect subtle differences in traffic behavior more effectively. However, normalizing per window can obscure broader trends and interactions that span across multiple windows, as each window is treated independently. In contrast, normalizing per trace involves scaling the packet counts across the entire trace before segmenting them into bins. This provides a uniform scale for all windows within a trace, preserving the relative differences across the entire connection. Normalizing per trace is advantageous for capturing long-term patterns and trends that persist throughout the trace. However, this may reduce sensitivity to short-term fluctuations, as the normalization is influenced by the extremes across the entire trace. Additionally, this form of normalization requires an offline analysis, making it unsuitable for online algorithms.


\textbf{Potential uses of the dataset:}
The proposed dataset offers significant value not only in the networking domain but also in the ML field. From a ML perspective, it provides a novel way to represent complex, real-world phenomena—such as network traffic—through images. As outlined in this work, these images can be generated with varying resolutions, enabling researchers to study how different levels of granularity affect the performance of DL models, particularly those designed for image recognition. This aspect of the dataset opens up opportunities to investigate the optimal image resolution required for detecting intricate patterns in network traffic. For instance, researchers could generate an image from a trace using a set of parameters, $\mathbb{X}$, and compare it with another image from the same trace, using a different set of parameters, $\mathbb{Y}$ (e.g., resolution, density, normalization). Another key contribution is the structured nature of the dataset. Based on real-world QUIC traffic traces, it exhibits characteristics not commonly found in standard datasets, such as significant class imbalance, with certain labels appearing at very low frequencies (e.g., as low as 0.001\%). Additionally, the dataset is well-suited for ordinal regression tasks, where the order of the labels is crucial. As demonstrated with our custom loss function (see \ref{LOSS}), predicting a label of 18 for a true value of 19 is closer to the correct answer than predicting 17 or 21, emphasizing the importance of maintaining label order. This unique structure makes the dataset valuable for exploring new methodologies and loss functions in ML research.

From a networking perspective, the contributions are even more direct. The dataset can be applied to a wide range of network-related analyses, from detecting DDoS attacks and traffic anomalies to examining symmetric and asymmetric flows, which could help identify the types of applications in use. It also holds promise for round-trip time (RTT) estimation and assisting load balancers in optimizing the distribution of network traffic, ultimately improving network management and performance.

==> sections/5-application.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{figforpaper/01-dataset-distribution-v5.pdf}
    \caption{Response distribution for training and evaluation datasets with a $T=0.1$-second sliding window.}
    \Description{Pie charts showing the response distribution for training and evaluation datasets with a $T=0.1$-second sliding window. Each chart displays percentages for various response classes, highlighting differences in class representation between training and test datasets.}
    \label{fig:response-distribution-dataset}
    % \label{fig:01-window-length}
\end{figure*}
We consider an observer who can see the encrypted QUIC packets transmitted between the client and the server. For each packet, the observer knows its direction, length, and observed time. Using this information, the QUIC traces can be converted into representative colored images suitable for training ML models. To convert the captured QUIC traces into time-series data, we use the sliding window technique~\citet{frank2001time}, which requires two configurable parameters: the window length and the overlap between consecutive windows. These images enable use cases like estimating HTTP/3 responses to aid load balancing.

Estimating the number of HTTP/3 responses in a QUIC connection can assist a load balancer in making more informed decisions. By monitoring connections and estimating the number of responses within each connection, the load balancer can determine if a connection is considered heavy and adjust its decision on the selected server accordingly~\cite{shahla2024trafficgrinder}. To evaluate the use of \textit{VisQUIC}, we formulate estimating the number of responses in a QUIC connection as a discrete regression problem and evaluate it using images derived from the traces. The dataset can be split into two settings: when the web servers are known to the observer and when they are not. We provide an evaluation for the case when the web servers are known to the observer. Therefore, the training and evaluation phases are conducted exclusively on the QUIC traces pertaining to the web servers assumed at inference time, using an $80:20$ train-test split to ensure out-of-sample evaluation. 
%Figure \ref{fig:response-distribution-dataset} in the Appendix shows the response distribution for training and evaluation datasets with two window lengths.

This is not a classic classification task because misclassification errors depend on the distance between predicted and actual categories. For example, estimating an image with $17$ responses as $16$ is better than estimating it as $15$ or $19$. It is also not a standard regression task, as the target categories are discrete. To address this issue, we developed a dedicated loss function coupled with data augmentation that: (1) accounts for the imbalanced dataset derived from real-world QUIC traces, and (2) rewards the model for correctly predicting classes closer to the actual label over those that are farther away. Appendix A.1 explains the discrete regression loss function in more detail.

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figforpaper/scatter_01_model_on01_traces.pdf}
        \caption{Window length $T=0.1$-sec}
        \Description{Scatter plot showing the predictive results for a window length of 0.1 second. Most points align along the perfect prediction line, with transparency applied to indicate overlapping densities.}
        \label{fig4:scatter_trace01}
    \end{subfigure}
    \hfill % optional; add some horizontal spacing
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figforpaper/scatter_03_model_on03_traces.pdf}
        \caption{Window length $T=0.3$-sec}
        \Description{Scatter plot showing the predictive results for a window length of 0.3 seconds. A higher density of points appears near the perfect prediction line, indicating accurate predictions.}
        \label{fig4:scatter_trace03}
    \end{subfigure}
    \caption{Scatter plots demonstrating the predictive results, where each point represents the summed predictions of a trace compared to its true label, with transparency set to $0.05$ to distinguish point density in overlapping areas.}
    \Description{Two scatter plots compare predictions against true labels for two different window lengths (0.1 and 0.3 seconds). Points closer to the red "Perfect Prediction" line indicate better prediction accuracy, and transparency highlights overlapping data densities.}
    \label{fig:traces-eval-images-03-model-03and01}
\end{figure}

We present a quantitative evaluation of the proposed framework when the web servers are known to the observer, using a subset of the dataset not included in training. Models were trained and evaluated exclusively on the QUIC traces pertaining to the web servers assumed at inference time. Two different models were trained with window lengths of $T=0.1$ and $T=0.3$ seconds. Classes with labels less than or equal to 20 constitute 90\% of the traces in the $T=0.3$-second window dataset and 95\% in the $T=0.1$-second window dataset. Due to their scarcity, classes above 20 were excluded from the training and test sets. While both $T=0.1$- and $T=0.3$-second sliding window datasets were created, we include only the response distribution for the $T=0.1$ dataset in Figure~\ref{fig:response-distribution-dataset} for brevity. The $T=0.3$ dataset exhibits similar trends, with slight variations in the distribution due to the larger window size. Figure \ref{fig:response-distribution-dataset} shows the images distribution for the created images datasets. 

% \begin{figure*}[htbp] % Added 'htbp' for better float placement
    % \centering
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.52\textwidth]{figforpaper/01-dataset-distribution-v5.pdf}
%     \caption{Response distribution for training and evaluation datasets with a $T=0.1$-second sliding window.}
%     \Description{Pie charts showing the response distribution for training and evaluation datasets with a $T=0.1$-second sliding window. Each chart displays percentages for various response classes, highlighting differences in class representation between training and test datasets.}
%     \label{fig:response-distribution-dataset}
%     % \label{fig:01-window-length}
% \end{figure}
    % \vspace{5mm} % Add consistent vertical spacing between subfigures
    % \begin{subfigure}{0.8\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figforpaper/03-dataset-distribution-v5.pdf}
    %     \caption{$T=0.3$ window dataset}
    %     \Description{Pie charts showing the response distribution for training and evaluation datasets with a $T=0.3$-second sliding window. The charts highlight the class frequency distributions and their variations between the datasets.}
    %     \label{fig:03-window-length}
    % \end{subfigure}
    % \caption{Response distribution for training and evaluation datasets with a $T=0.1$-second sliding window.}
    % \Description{The figure consists of two subfigures, each showing pie charts for training and evaluation datasets. The first subfigure represents the $T=0.1$-second window dataset, while the second represents the $T=0.3$-second window dataset. Each pie chart shows the percentage of responses per class, allowing for visual comparison of class distributions between datasets and window lengths.}
    % \label{fig:response-distribution-dataset}
% \end{figure*}


%Both datasets are significantly skewed. As the figure demonstrates, images whose class values are $10$ or more are infrequent in both datasets. In the $T=0.1$-second window dataset, labels $0,1$ and $2$ make up roughly $75\%$ of the data, with the higher classes being represented in smaller proportions. Conversely, in the $T=0.3$-second window dataset, there is a more even distribution, with labels $0,1$ and $2$ comprising only about $47\%$ of the total dataset. \textcolor{red}{Maybe we need to say again here why we omitted above 20}

To address class imbalance, we developed a dedicated loss function and implemented a data augmentation technique. A grid search was used to optimize loss function parameters $\alpha$, $\beta$, and $\gamma$, with $\alpha \in {0.3, 0.5, 0.7}$, $\beta \in {0.4, 0.6}$, and $\gamma \in {1, 2, 3}$. The optimal values, selected based on the lowest validation loss during training, were $\alpha=0.7$, $\beta=0.4$, and $\gamma=2$ for $T=0.3$ seconds, and $\gamma=3$ for $T=0.1$ seconds with the same $\alpha$ and $\beta$. Data augmentation was applied selectively to minority classes (values $10$–$20$) since the $32 \times 32$ pixel grids, derived from QUIC traces, encode temporal dependencies that non-order-preserving modifications could disrupt. Therefore, we introduced minimal noise with a standard deviation of $\sigma=2.55$ (1\% of pixel value), preserving temporal integrity while enhancing model robustness and generalization~\cite{maharana2022review}. Training was performed with a batch size of 64 images using the Adam optimizer~\cite{kingma2014adam} and the ReduceLROnPlateau learning rate scheduler, reducing the learning rate by 30\% when a plateau was detected, with an early stopping technique. 
%The performance is measured on an AMD Ryzen Threadripper PRO 3955WX 16C CPU 3.9G running at 64MB cache, 64GB of CRUCIAL CT8G4DFRA32A RAM clocked at 3200MHz and an NVIDIA GTX-4090 GPU.

The results presented are for estimating the total number of HTTP/3 responses in a complete trace. The images were fed sequentially through the trained models, whose predictions were summed and compared to the sum of the trace's true labels. Figure~\ref{fig:traces-eval-images-03-model-03and01} shows prediction results using the evaluation traces with the $T=0.1$- and $T=0.3$-second subdivisions.

In these scatter plots, the parameter $\theta$, ranging between 0 and 1, modulates the transparency of the points. We set $\theta$ to $0.05$ to enhance visual distinction between areas of high and low point density among the roughly $12,000$ data points. Each point represents the summed predictions over the images of a trace compared to its true label. For example, if a trace is composed of five non-overlapping images with true labels 1, 0, 2, 4, and 1 (totaling 8), and the model's predictions are 1, 0, 3, 4, and 1 (totaling 9), the trace is represented at the point (8, 9) in the plot. Overlapping points become darker due to the transparency setting.

Additionally, we introduce a Cumulative Accuracy Profile (CAP) metric, which provides a refined measure of classification accuracy by incorporating a tolerance level for each prediction. Unlike traditional metrics such as confusion matrices that require exact matches between predicted and true labels, CAP allows for a specified degree of tolerance, accommodating predictions that are close to the correct class. Formally, it is defined as: $\mathrm{CAP}_{\pm k}(\mathbf{y}, \hat{\mathbf{y}}) = \frac{1}{n} \sum_{i=1}^n \mathbf{\mathbb{1}}(|y_i - \hat{y}_i| \leq k),$ where \( \mathbf{y} \) represents the vector of true class labels, \( \hat{\mathbf{y}} \) denotes the model’s predictions, \( k \) specifies the tolerance level (e.g., \(\pm 1\) or \(\pm 2\) classes), \( n \) is the total number of samples, and \( \mathbb{1}(\cdot) \) is the indicator function that evaluates to $1$ if the condition is met and $0$ otherwise. This metric thus quantifies the proportion of samples where the model’s predictions fall within the allowed tolerance around the true class.

Figure~\ref{fig:traces-eval-images-03-model-03and01}(\subref{fig4:scatter_trace01}) shows the scatter plot for predictions from the model trained using $T=0.1$-second window images, while Figure~\ref{fig:traces-eval-images-03-model-03and01}(\subref{fig4:scatter_trace03}) displays results for the $T=0.3$-second window. The test dataset includes $12,520$ traces with an average of $21.2$ images per trace for $T=0.1$ seconds, and $12,142$ traces with an average of $7.5$ images per trace for $T=0.3$ seconds.

The figures highlight significant differences in performance between the two models. The $T=0.3$-second model has 71\% of predictions within $\pm3$ (CAP) of the true values, whereas the $T=0.1$-second model achieves 92.6\%, demonstrating a nearly 20\% improvement in accuracy. We use a $\pm3$ tolerance level because, for both window lengths, the points represent aggregated prediction sums and, thus, aggregated errors. Additionally, the predictions of the model trained using a $T=0.1$-second window are more closely aligned along the diagonal, showing less deviation compared to those of the $T=0.3$-second model, suggesting that finer timing resolutions enhance cumulative prediction performance.

Figures \ref{fig:traces-eval-images-03-model-03and01}(\subref{fig4:scatter_trace01}) and \ref{fig:traces-eval-images-03-model-03and01}(\subref{fig4:scatter_trace03}) illustrate notable differences in predictive behavior between models trained and evaluated with $T=0.3$-second and $T=0.1$-second window sizes. Specifically, diagonal patterns appear in the predictions of the $T=0.3$-second model that are absent in the $T=0.1$-second model's predictions. This phenomenon exists for several reasons. When using a $T=0.1$ subdivision, a high percentage of images have lower class values, and the model trained on this dataset is very accurate for low-value classes. In contrast, a $T=0.3$ subdivision yields images with higher class values, increasing the variance of the true labels, and both models perform worse for higher-value classes compared to lower-value ones. Additionally, any incorrect prediction by either model contributes to an increase in the cumulative predictions for the remainder of the trace, thereby elevating the overall predicted values. The $T=0.1$-second model's box plot is presented in Appendix.

==> sections/VISQUIC-reorgainize.tex <==
\section{VisQUIC}
In this section, we introduce the \textit{VisQUIC} dataset, a comprehensive collection of QUIC traffic traces gathered over a four-month period, accompanied by SSL keys to enable thorough analysis of encrypted QUIC traffic.

\subsection{Dataset Collection}
The process starts with HTTP/3~\citep{rfc9114} GET requests that are generated to various web servers that support HTTP/3. The websites were selected from the Tranco list~\citep{tranco}, which provides a reliable ranking of the most visited domains. Data collection was performed from two residential networks across different continents, with collection conducted over a four-month period throughout all the days. This temporal and geographical diversity helps capture how QUIC traffic patterns vary under different network conditions and server distances.

To ensure consistent experimental conditions and minimize noise in the collected data, we use Headless Chrome~\citep{headless} version 119.0.6046.159 in incognito mode with the application cache disabled. This choice deliberately creates a controlled environment where each connection maintains identical baseline conditions. The network traffic traces are captured using Tshark~\citep{merino2013instant} in packet capture (PCAP) format, containing only QUIC packets that cover the duration of the website request.

\subsection{Dataset Components}
The \textit{VisQUIC} dataset consists of three main components. The core of our dataset comprises over 100,000 QUIC traces collected from more than 44,000 websites. For each PCAP file, we provide the corresponding SSL keys used to encrypt the traffic, enabling researchers to decrypt and analyze the content of QUIC connections. This combination of encrypted traces and keys allows for comprehensive analysis of QUIC's behavior and performance characteristics.

Table~\ref{tab:combined-table1} presents detailed statistics about the dataset, showing the distribution of traces across different web servers. The dataset includes traffic from various services, each exhibiting different traffic characteristics and implementation patterns.

\begin{table}
\caption{Summary statistics of QUIC traces and the number of images per dataset for each web server.}
% \tiny
% \small
\begin{tabular}{|p{2.2cm}|p{1.3cm}|p{0.9cm}|p{1.2cm}|c|}
\hline
\centering \textbf{Web Server} & \centering \textbf{Websites} & \centering \textbf{Traces} & \centering \textbf{$T=0.1$} & \textbf{$T=0.3$} \\ \hline
\centering youtube & \centering 399 & \centering 2,109 & \centering 139,889 & 54,659 \\ \hline
\centering semrush & \centering 1,785 & \centering 9,489 & \centering 474,716 & 221,477 \\ \hline
\centering discord & \centering 527 & \centering 7,271 & \centering 623,823 & 235,248 \\ \hline
\centering instagram & \centering 3 & \centering 207 & \centering 17,003 & 7,112 \\ \hline
\centering mercedes-benz & \centering 46 & \centering 66 & \centering 9,987 & 2,740 \\ \hline
\centering bleacherreport & \centering 1,798 & \centering 8,497 & \centering 781,915 & 331,530 \\ \hline
\centering nicelocal & \centering 1,744 & \centering 1,666 & \centering 148,254 & 48,900 \\ \hline
\centering facebook & \centering 13 & \centering 672 & \centering 25,919 & 10,988 \\ \hline
\centering pcmag & \centering 5,592 & \centering 13,921 & \centering 1,183,717 & 385,797 \\ \hline
\centering logitech & \centering 177 & \centering 728 & \centering 56,792 & 28,580 \\ \hline
\centering google & \centering 1,341 & \centering 2,149 & \centering 81,293 & 29,068 \\ \hline
\centering cdnetworks & \centering 902 & \centering 2,275 & \centering 207,604 & 85,707 \\ \hline
\centering independent & \centering 3,340 & \centering 3,453 & \centering 176,768 & 68,480 \\ \hline
\centering cloudflare & \centering 26,738 & \centering 44,700 & \centering 1,347,766 & 341,488 \\ \hline
\centering jetbrains & \centering 35 & \centering 1,096 & \centering 34,934 & 18,470 \\ \hline
\centering pinterest & \centering 43 & \centering 238 & \centering 6,465 & 2,360 \\ \hline
\centering wiggle & \centering 4 & \centering 0 & \centering 0 & 0 \\ \hline
\centering cnn & \centering 27 & \centering 2,127 & \centering 91,321 & 59,671 \\ \hline
\end{tabular}
\label{tab:combined-table1}
\end{table}

We filtered our dataset in two stages. First, we removed non-QUIC packets from the raw traffic captures. Then, we identified and removed duplicate images (to be elaborated later in the paper) that resulted from identical traffic patterns, reducing the dataset from $21,100,925$ to $5,040,459$ images. While our raw dataset contains all captured responses, images with more than 20 responses were excluded from training and evaluation due to their extreme rarity in real-world traffic. \footnote{The captured traces, images, and code will be available upon the paper's acceptance using a GitHub link.}

\subsection{Supplementary Features}
To support machine learning applications, we provide additional tools and features alongside the core dataset. While our primary contribution is the QUIC traffic dataset, we also provide tools for converting traffic patterns into visual representations. Following established approaches~\citep{farrukh2023senet, golubev2022image, shapira2019flowpic, tobiyama2016malware, velan2015survey}, these tools can transform network features such as packet timing, sizes, and directions into RGB images.

The image generation process begins with data extraction, where we collect packet metadata including arrival time, length, and direction information. These features are then organized through time and length binning, where the trace's time span is divided into equispaced bins. A histogram construction phase follows, counting packets in each bin based on their characteristics. The final step maps these counts to pixel intensities in an RGB image, with the red channel representing server-to-client packets and the green channel representing client-to-server packets, while the blue channel remains unused.

\begin{figure}[t] 
\centering 
\includegraphics[width=0.9\linewidth]{figforpaper/image-construction.pdf} 
\caption{Construction of an image from a QUIC trace, illustrating how QUIC traffic patterns are transformed into visual features. Raw packet metadata captures timing, size, and directional information, which is then binned by time and length, creating separate histograms for client-to-server (green) and server-to-client (red) traffic. The histogram peaks indicate bursts of activity, common in HTTP/3 request-response patterns. The final RGB representation preserves temporal relationships and traffic directionality, where pixel intensity indicates packet density and color indicates direction.}
\Description{The figure demonstrates the process of constructing an image from a QUIC trace. It shows three steps: the extraction of time-series statistics, binning packets by time and length into histograms, and mapping the data into an RGB image with green and red intensities representing different directions of traffic.}
\label{fig:image-const} 
\end{figure}

For traffic labeling, we provide various characteristics extracted from the decrypted traces, including the number of HTTP/3 responses within different time windows. These labels can serve as ground truth for supervised learning tasks, though researchers are free to generate alternative labels based on their specific research needs.

\subsection{Dataset Characteristics and Coverage}
The dataset's temporal characteristics are particularly notable in two key aspects. Our window-based approach uses two different timescales ($T=0.1$ and $T=0.3$ seconds) to capture traffic patterns at different granularities, enabling the study of both micro-level interactions and broader connection behaviors. Additionally, the class distribution of HTTP/3 responses exhibits a natural long-tail pattern, with fewer instances of high-response scenarios, providing researchers with realistic traffic patterns for analysis.

This comprehensive dataset enables researchers to study QUIC traffic patterns across different services, analyze protocol behavior under varying network conditions, develop machine learning models robust to class imbalance and temporal dependencies, and investigate HTTP/3 multiplexing patterns in real-world scenarios. The combination of raw traces, SSL keys, and supplementary tools provides a flexible foundation for a wide range of QUIC and HTTP/3 research.

The effect of resolution choice on traffic visualization becomes apparent when examining traces at different pixel densities. Figure~\ref{fig:different-responses1} demonstrates how increasing resolution affects the representation of traffic patterns. At lower resolutions of $16 \times 16$, traffic patterns appear as aggregate flows where overlapping client and server activities create yellow pixels. As the resolution increases to $32 \times 32$ and $64 \times 64$, these overlapped regions separate into distinct red and green components, revealing more detailed timing relationships between requests and responses. The higher resolutions of $128 \times 128$ and $256 \times 256$ capture fine-grained packet interactions, though at increased computational cost.

\begin{figure}[htbp]
   \centering
   \begin{subfigure}{0.15\textwidth}
       \centering
       \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-16.png}
       \caption{$16 \times 16$}
       \Description{An image representation of a QUIC flow using a $16 \times 16$ resolution. The image contains sparse colored pixels indicating packet activities.}
       \label{fig:161}
   \end{subfigure}%
   \hfill
   \begin{subfigure}{0.15\textwidth}
       \centering
       \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-32.png}
       \caption{$32 \times 32$}
       \Description{An image representation of a QUIC flow using a $32 \times 32$ resolution. The image has increased pixel density compared to the $16 \times 16$ version, with clearer representation of packet activities.}
       \label{fig:321}
   \end{subfigure}%
   \hfill
   \begin{subfigure}{0.15\textwidth}
       \centering
       \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-64.png}
       \caption{$64 \times 64$}
       \Description{An image representation of a QUIC flow using a $64 \times 64$ resolution. The pixel density increases, providing finer details of the packet activities.}
       \label{fig:641}
   \end{subfigure} 
   \vspace{1mm}
   \begin{subfigure}{0.23\textwidth}
       \centering
       \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-128.png}
       \caption{$128 \times 128$}
       \Description{An image representation of a QUIC flow using a $128 \times 128$ resolution. The pixel density further increases, capturing more detailed packet activities.}
       \label{fig:1281}
   \end{subfigure}%
   \hfill
   \begin{subfigure}{0.23\textwidth}
       \centering
       \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-256.png}
       \caption{$256 \times 256$}
       \Description{An image representation of a QUIC flow using a $256 \times 256$ resolution. This high-resolution image provides the most detailed representation of packet activities.}
       \label{fig:2561}
   \end{subfigure}
   \caption{Impact of resolution on QUIC traffic visualization using $T=0.1$-second windows. Lower resolutions show aggregate traffic patterns, while higher resolutions reveal detailed temporal and directional relationships between packets.}
   \Description{The figure presents five images of a QUIC flow at resolutions of $16 \times 16$, $32 \times 32$, $64 \times 64$, $128 \times 128$, and $256 \times 256$. Each image captures the packet activity within a $0.1$-second window, with increasing detail as resolution increases.}
   \label{fig:different-responses1}
\end{figure}

When normalizing the packet counts in these visualizations, we considered both per-window and per-trace approaches. Per-window normalization highlights short-term variations in traffic patterns, making it easier to detect subtle differences in packet behavior within each time window. Conversely, per-trace normalization maintains consistent scaling across an entire connection, better preserving long-term patterns but potentially reducing sensitivity to short-term fluctuations. Our dataset includes both normalization options, allowing researchers to choose the approach that best suits their analysis needs.

The \textit{VisQUIC} dataset is made publicly available to the research community, providing a valuable resource for advancing studies in QUIC, HTTP/3, and encrypted traffic analysis. The combination of raw traces, SSL keys, and supplementary visualization tools enables researchers to explore various aspects of QUIC behavior, from protocol-level interactions to high-level traffic patterns. Details for accessing the dataset are available at [Dataset Website/Repository].

==> sections/VisQUICDataset.tex <==
In this section, we introduce the \textit{VisQUIC} dataset, a comprehensive collection of QUIC traffic traces accompanied by SSL keys and image representations, designed to facilitate advanced research in network analysis and ML.

\subsection{Dataset Collection and Generation}
The process starts with HTTP/3~\citep{rfc9114} GET requests that are generated to various web servers that support HTTP/3, each hosting multiple websites. Requests are issued for up to 26,000 different websites per web server. Headless Chrome~\citep{headless} is used in incognito mode with the application cache disabled, and the websites are requested sequentially, resulting in a web-page request workload. Table~\ref{tab:combined-table1} displays the exact numbers for each web server and more detailed statistics broken down per web server for each class are provided in Appendix A.3. The generated network traffic traces are captured using Tshark~\citep{merino2013instant} in packet capture (PCAP) format. These traces include only QUIC packets and cover the duration of the website request. For each PCAP file the corresponding SSL keys are stored to be used later to decrypt the traffic. The SSL keys are also provided in the dataset's materials.

\subsection{Image Generation Technique}
To transform the network traffic data into a format suitable for ML models, we converted the captured traces into images. This process involves representing features such as packet arrival times, packet sizes, packet density, and packet directions as visual elements in an image. The use of images enhances pattern recognition abilities~\citep{farrukh2023senet, golubev2022image, shapira2019flowpic, tobiyama2016malware, velan2015survey}, allowing deep learning models to identify intricate patterns in network traffic.

Figure~\ref{fig:image-const} illustrates the steps involved in constructing an image from a trace:
\begin{enumerate} 
    \item \textbf{Data Extraction:} Collect packet metadata including arrival time, length, and direction (client-to-server and server-to-client). 
    \item \textbf{Time and Length Binning:} Divide the time span of the trace into $M$ equispaced time bins and the packet lengths into $N$ bins. 
    \item \textbf{Histogram Construction:} Count the number of packets in each bin based on time and length, separately for each direction. 
    \item \textbf{Image Creation:} Map the histogram counts to pixel intensities in an RGB image, with the red channel representing server-to-client packets and the green channel representing client-to-server packets. The blue channel remains unused.    
\end{enumerate}

This technique extends the FlowPic method~\citep{shapira2019flowpic} by incorporating directional information and configurable parameters such as window length and resolution. FlowPic’s single-channel approach, while providing a general traffic overview, is insufficient in the context of QUIC. In QUIC, distinguishing between client-to-server and server-to-client traffic is critical due to the multiplexed nature of HTTP/3 requests and responses. Furthermore, QUIC’s inherent complexity—stemming from stream multiplexing and independent packet handling—necessitates a more detailed examination of traffic directions. For those reasons, we introduce a separate channel for each direction between a client and a server, a density factor for the packets' count in a given window, and a configurable number of bins.

\begin{figure}[t] 
\centering \includegraphics[width=0.9\linewidth]{figforpaper/image-construction.pdf} 
\caption{Construction of an image from a QUIC trace. Packet metadata is binned by time and length, and mapped to pixel intensities resulting in an RGB image.}
\Description{The figure demonstrates the process of constructing an image from a QUIC trace. It shows three steps: the extraction of time-series statistics, binning packets by time and length into histograms, and mapping the data into an RGB image with green and red intensities representing different directions of traffic.}
\label{fig:image-const} 
\end{figure}

Images whose class labels were above 20 responses were not part of the training or evaluation for estimating the number of responses in a QUIC connection, due to their rarity in the data. Besides that, the raw data contains all of the data, unfiltered. Preprocessing was done by filtering out packets that are not QUIC packets. Furthermore, a large number of images were identical, and all of the duplicate images were removed. Before the filtering there was $21,100,925$ images, and after there was $5,040,459$ images. We upload the full dataset including the duplicates. \footnote{The captured traces, images, and code will be available upon the paper's acceptance using a GitHub link.}

The \textit{VisQUIC} dataset includes three main components: trace data, image data, and labels. The \textbf{trace data} comprises over 100,000 QUIC traces collected from more than 44,000 websites. For each trace, the corresponding SSL keys are provided to enable decryption, allowing in-depth analysis of the encrypted traffic.
The \textbf{image data} consists of over seven million images generated from the traces. These images are created using two different window lengths, $T=0.1$ seconds and $T=0.3$ seconds, capturing network traffic at varying temporal resolutions. The images have a resolution of $M=N=32$, which balances the level of detail captured with computational efficiency, making them suitable for ML applications. Each image can be associated with \textbf{labels}, such as the number of HTTP/3 requests or responses observed during the captured window. These labels are derived using the SSL keys to decrypt the traces and extract relevant metadata. This labeling enables the dataset to be used for supervised learning tasks, facilitating research in network traffic analysis and ML. Table \ref{tab:combined-table1} present \textit{VisQUIC}'s characteristics.

\begin{table}
\caption{Summary statistics of QUIC traces and the number of images per dataset for each web server.}
% \tiny
% \small
\begin{tabular}{|p{2.2cm}|p{1.3cm}|p{0.9cm}|p{1.2cm}|c|}
\hline
\centering \textbf{Web Server} & \centering \textbf{Websites} & \centering \textbf{Traces} & \centering \textbf{$T=0.1$} & \textbf{$T=0.3$} \\ \hline
\centering youtube & \centering 399 & \centering 2,109 & \centering 139,889 & 54,659 \\ \hline
\centering semrush & \centering 1,785 & \centering 9,489 & \centering 474,716 & 221,477 \\ \hline
\centering discord & \centering 527 & \centering 7,271 & \centering 623,823 & 235,248 \\ \hline
\centering instagram & \centering 3 & \centering 207 & \centering 17,003 & 7,112 \\ \hline
\centering mercedes-benz & \centering 46 & \centering 66 & \centering 9,987 & 2,740 \\ \hline
\centering bleacherreport & \centering 1,798 & \centering 8,497 & \centering 781,915 & 331,530 \\ \hline
\centering nicelocal & \centering 1,744 & \centering 1,666 & \centering 148,254 & 48,900 \\ \hline
\centering facebook & \centering 13 & \centering 672 & \centering 25,919 & 10,988 \\ \hline
\centering pcmag & \centering 5,592 & \centering 13,921 & \centering 1,183,717 & 385,797 \\ \hline
\centering logitech & \centering 177 & \centering 728 & \centering 56,792 & 28,580 \\ \hline
\centering google & \centering 1,341 & \centering 2,149 & \centering 81,293 & 29,068 \\ \hline
\centering cdnetworks & \centering 902 & \centering 2,275 & \centering 207,604 & 85,707 \\ \hline
\centering independent & \centering 3,340 & \centering 3,453 & \centering 176,768 & 68,480 \\ \hline
\centering cloudflare & \centering 26,738 & \centering 44,700 & \centering 1,347,766 & 341,488 \\ \hline
\centering jetbrains & \centering 35 & \centering 1,096 & \centering 34,934 & 18,470 \\ \hline
\centering pinterest & \centering 43 & \centering 238 & \centering 6,465 & 2,360 \\ \hline
\centering wiggle & \centering 4 & \centering 0 & \centering 0 & 0 \\ \hline
\centering cnn & \centering 27 & \centering 2,127 & \centering 91,321 & 59,671 \\ \hline
\end{tabular}
\label{tab:combined-table1}
\end{table}
% \begin{table}
% \caption{Summary statistics of QUIC traces and the number of images per dataset for each web server.}
% % \tiny
% % \small
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% \textbf{Web Server} & \textbf{Websites} & \textbf{Traces} & \textbf{$T=0.1$} & \textbf{$T=0.3$} \\ \hline
% youtube.com & 399 & 2,109 & 139,889 & 54,659 \\ \hline
% semrush.com & 1,785 & 9,489 & 474,716 & 221,477 \\ \hline
% discord.com & 527 & 7,271 & 623,823 & 235,248 \\ \hline
% instagram.com & 3 & 207 & 17,003 & 7,112 \\ \hline
% mercedes-benz.com & 46 & 66 & 9,987 & 2,740 \\ \hline
% bleacherreport.com & 1,798 & 8,497 & 781,915 & 331,530 \\ \hline
% nicelocal.com & 1,744 & 1,666 & 148,254 & 48,900 \\ \hline
% facebook.com & 13 & 672 & 25,919 & 10,988 \\ \hline
% pcmag.com & 5,592 & 13,921 & 1,183,717 & 385,797 \\ \hline
% logitech.com & 177 & 728 & 56,792 & 28,580 \\ \hline
% google.com & 1,341 & 2,149 & 81,293 & 29,068 \\ \hline
% cdnetworks.com & 902 & 2,275 & 207,604 & 85,707 \\ \hline
% independent.co.uk & 3,340 & 3,453 & 176,768 & 68,480 \\ \hline
% cloudflare.com & 26,738 & 44,700 & 1,347,766 & 341,488 \\ \hline
% jetbrains.com & 35 & 1,096 & 34,934 & 18,470 \\ \hline
% pinterest.com & 43 & 238 & 6,465 & 2,360 \\ \hline
% wiggle.com & 4 & 0 & 0 & 0 \\ \hline
% cnn.com & 27 & 2,127 & 91,321 & 59,671 \\ \hline
% \end{tabular}
% \label{tab:combined-table1}
% \end{table}

\subsection{Discussion}
When generating images for the \textit{VisQUIC} dataset, the choice of parameters significantly influences their effectiveness for analysis.

\textbf{Window Length ($T$):} The window length determines the temporal span of each image and affects data granularity. Shorter windows capture detailed interactions but increase computational demands due to more images, while longer windows provide an aggregated view, reducing image count but potentially obscuring fine-grained details.

\textbf{Image Resolution:} Resolution balances detail and computational efficiency. Higher resolutions capture finer features but increase resource requirements. The resolution should align with the analysis goals and computational constraints.

\textbf{Normalization Approach:} Normalization impacts outcomes by scaling packet counts. Per-window normalization highlights short-term variations, aiding detection of subtle differences, while per-trace normalization captures long-term patterns but may reduce sensitivity to short-term fluctuations. The choice depends on specific analysis needs.

\textbf{Choosing Image Parameters:} Figure \ref{fig:different-responses1} illustrates the effect of resolution on image representation. At lower resolutions (e.g., Figure \ref{fig:different-responses1}(\subref{fig:161})), a yellow pixel combines packets from both directions (red and green channels). Increasing resolution (Figures \ref{fig:different-responses1}(\subref{fig:321}) and \ref{fig:different-responses1}(\subref{fig:641})) splits these into separate red or green pixels, providing finer granularity and more detailed insights into packet interactions.
\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-16.png}
        \caption{$16 \times 16$}
        \Description{An image representation of a QUIC flow using a $16 \times 16$ resolution. The image contains sparse colored pixels indicating packet activities.}
        \label{fig:161}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-32.png}
        \caption{$32 \times 32$}
        \Description{An image representation of a QUIC flow using a $32 \times 32$ resolution. The image has increased pixel density compared to the $16 \times 16$ version, with clearer representation of packet activities.}
        \label{fig:321}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-64.png}
        \caption{$64 \times 64$}
        \Description{An image representation of a QUIC flow using a $64 \times 64$ resolution. The pixel density increases, providing finer details of the packet activities.}
        \label{fig:641}
    \end{subfigure} 
    \vspace{1mm}
    \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-128.png}
        \caption{$128 \times 128$}
        \Description{An image representation of a QUIC flow using a $128 \times 128$ resolution. The pixel density further increases, capturing more detailed packet activities.}
        \label{fig:1281}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-256.png}
        \caption{$256 \times 256$}
        \Description{An image representation of a QUIC flow using a $256 \times 256$ resolution. This high-resolution image provides the most detailed representation of packet activities.}
        \label{fig:2561}
    \end{subfigure}
    \caption{Five example images of QUIC flows using $T=0.1$-second windows with different pixel levels.}
    \Description{The figure presents five images of a QUIC flow at resolutions of $16 \times 16$, $32 \times 32$, $64 \times 64$, $128 \times 128$, and $256 \times 256$. Each image captures the packet activity within a $0.1$-second window, with increasing detail as resolution increases.}
    \label{fig:different-responses1}
\end{figure}

\subsection{Potential Applications of the Dataset}

\textit{VisQUIC} offers significant value in both networking and ML domains by enabling the analysis of QUIC and HTTP/3 behavior under real-world conditions. Researchers can leverage the comprehensive data provided by the dataset to develop tools and methodologies that enhance network performance and advance ML techniques.

From a \textbf{networking} perspective, the dataset assists in detecting DDoS attacks and traffic anomalies, which is crucial for maintaining network security and reliability. It enables the examination of symmetric and asymmetric flows to identify application types, aiding in effective traffic management. Additioanly, estimating round-trip times (RTT) helps ISPs monitor their network performance and manage it accordingly, and lastly estimating the number of responses in a connection a load balancer. The dataset also  facilitates to studies on encrypted traffic patterns, congestion control mechanisms, and protocol performance, which are essential for understanding and enhancing modern network communications.

From an \textbf{ML} perspective, the dataset allows for the exploration of image-based representations of network traffic for classification and regression tasks. Researchers can study the effects of different image resolutions on deep learning model performance, providing insights into optimizing models for various applications. The dataset supports the investigation of methods for handling significant class imbalances and ordinal regression tasks, addressing common challenges in ML with real-world data. Furthermore, it offers opportunities to develop new loss functions tailored to the unique structure of the dataset.

\textbf{Dataset Accessibility}
\textit{VisQUIC} is made publicly available to the research community, providing a valuable resource for advancing studies in QUIC, HTTP/3, and related areas. Details on accessing the dataset are provided on \url{[Dataset Website/Repository]} upon request.

%\textbf{Potential Uses of the Dataset:}
%From a networking perspective, the dataset can be applied to a wide range of analyses, including:
%\begin{itemize} \item Detecting DDoS attacks and traffic anomalies. \item Examining symmetric and asymmetric flows to identify application types. \item Estimating round-trip times (RTT) and assisting load balancers in optimizing traffic distribution. \end{itemize}
%From a ML perspective, the dataset provides opportunities to:
%\begin{itemize} \item Study the effects of different image resolutions on deep learning model performance. \item Explore methods for handling significant class imbalances and ordinal regression tasks. \item Develop new methodologies and loss functions tailored to the unique structure of the dataset. \end{itemize}

%\subsection{Potential Applications}
%\textit{VisQUIC} offers significant value in both networking and ML domains. From a \textbf{networking} perspective, it enables the analysis of QUIC and HTTP/3 behavior under real-world conditions. Researchers can develop tools for traffic analysis, intrusion detection, and network performance optimization by leveraging the comprehensive data provided by the dataset. Specifically, the dataset can be applied to a wide range of analyses, including detecting DDoS attacks and traffic anomalies, examining symmetric and asymmetric flows to identify application types, and estimating round-trip times (RTT) to assist load balancers in optimizing traffic distribution. Additionally, it facilitates studies on encrypted traffic patterns, congestion control mechanisms, and protocol performance, which are crucial for understanding and improving modern network communications.

%From a \textbf{ML} perspective, the dataset allows for the exploration of image-based representations of network traffic for classification and regression tasks. It supports the investigation of deep learning models on complex, real-world datasets with class imbalances, providing opportunities to address challenges associated with imbalanced data. Researchers can study the effects of different image resolutions on deep learning model performance, explore methods for handling significant class imbalances and ordinal regression tasks, and develop new methodologies and loss functions tailored to the unique structure of the dataset. The dataset's unique characteristics make it valuable for advancing ML techniques in the context of network traffic analysis.


==> sections/VisQUICDataset1.tex <==
\textit{VisQUIC} is a large-scale dataset designed to facilitate benchmarking and research in encrypted traffic analysis. It contains over \textbf{100,000 labeled QUIC traces} collected from \textbf{44,000+ websites} over a four-month period. Unlike existing datasets, \textit{VisQUIC} provides \textbf{SSL keys} to enable controlled decryption, making it a unique resource for studying encrypted QUIC traffic. Additionally, \textit{VisQUIC} supports an optional image-based representation, allowing machine learning researchers to explore novel approaches for encrypted traffic analysis.

\subsection{Dataset Collection and Structure}
To ensure broad coverage, we collected QUIC traces from two residential networks across different continents, capturing diverse network conditions and geographical variations. Data collection was conducted throughout all hours of the day, enabling analysis of traffic behavior under varying load conditions.

The dataset was built using active probing of websites that support HTTP/3, selected from the Tranco list~\citep{tranco}, a reliable ranking of the most visited domains. We used \textbf{Headless Chrome}~\citep{headless} in incognito mode with caching disabled to ensure consistency across requests. Each website was requested sequentially, ensuring that every QUIC connection was independent of previous traffic. This methodology eliminates caching effects and session resumption artifacts, allowing for a clean and reproducible dataset.

To better capture general web traffic, the dataset focuses on traces from sequential web page requests rather than video streaming. The decision to prioritize page requests stems from the limited number of web servers that stream video over QUIC, which restricts server-side traffic diversity. In contrast, web page requests reflect a broader range of application-layer interactions, encompassing various content types, third-party services, and server-side behaviors. Furthermore, video streaming traffic is heavily influenced by adaptive bitrate algorithms and buffering mechanisms controlled by the server, making it less dependent on network conditions. By focusing on web page requests, the dataset provides a more representative view of how QUIC operates across different web services.

While \textit{VisQUIC} currently emphasizes web page traffic, future work should explore dataset extensions that incorporate varying bandwidth conditions, mobile network scenarios, and additional browsers beyond Chrome. Such extensions would provide a more comprehensive understanding of QUIC traffic across diverse environments.

\textbf{Traffic Capture and Encryption Data.}  
QUIC traffic was captured using \textbf{Tshark}~\citep{merino2013instant} in \textbf{packet capture (PCAP)} format, retaining only QUIC packets to focus on encrypted traffic analysis. Each PCAP file is accompanied by its corresponding \textbf{SSL keys}, allowing controlled decryption for research requiring payload inspection.

\subsection{Optional Image-Based Representation for ML Research}
In addition to raw network traces, \textit{VisQUIC} provides an \textbf{optional image-based representation} to support machine learning applications. This approach builds upon prior work on network traffic visualization~\citep{shapira2019flowpic, golubev2022image}, enhancing existing methods by introducing an RGB-based representation that encodes packet arrival times, sizes, and directions. Unlike previous work, which primarily relied on single-channel grayscale representations, our method leverages separate color channels to differentiate between client-to-server and server-to-client traffic. This enhancement preserves crucial directional and temporal relationships, making it particularly effective for analyzing HTTP/3 multiplexing patterns within QUIC traffic.

\begin{figure}[t] 
\centering \includegraphics[width=1\linewidth]{figforpaper/image-construction.pdf} 
\caption{Construction of an image from a QUIC trace. (a) Raw packet metadata captures timing, size, and directional information. (b) Packets are binned by time and length, creating histograms for client-to-server (green) and server-to-client (red) traffic. (c) The final RGB representation preserves temporal relationships and directionality, where pixel intensity indicates packet density.}
\label{fig:image-const} 
\end{figure}

To further illustrate the impact of different image resolutions, Figure~\ref{fig:different-resolutions} compares image representations of QUIC flows at varying pixel levels. Lower resolutions, such as $16 \times 16$, aggregate packet-level details, making them computationally efficient but potentially losing finer granularity. Conversely, higher resolutions (e.g., $256 \times 256$) preserve intricate temporal patterns but increase computational overhead.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-16.png}
        \caption{$16 \times 16$}
        \Description{An image representation of a QUIC flow using a $16 \times 16$ resolution. The image contains sparse colored pixels indicating packet activities.}
        \label{fig:161}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-32.png}
        \caption{$32 \times 32$}
        \Description{An image representation of a QUIC flow using a $32 \times 32$ resolution. The image has increased pixel density compared to the $16 \times 16$ version, with clearer representation of packet activities.}
        \label{fig:321}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-64.png}
        \caption{$64 \times 64$}
        \Description{An image representation of a QUIC flow using a $64 \times 64$ resolution. The pixel density increases, providing finer details of the packet activities.}
        \label{fig:641}
    \end{subfigure} 
    \vspace{1mm}
    \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-128.png}
        \caption{$128 \times 128$}
        \Description{An image representation of a QUIC flow using a $128 \times 128$ resolution. The pixel density further increases, capturing more detailed packet activities.}
        \label{fig:1281}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figforpaper/business-google-00780-L01-N36-256.png}
        \caption{$256 \times 256$}
        \Description{An image representation of a QUIC flow using a $256 \times 256$ resolution. This high-resolution image provides the most detailed representation of packet activities.}
        \label{fig:2561}
    \end{subfigure}
        \caption{Comparison of QUIC image representations at different resolutions. The lower resolution loses finer packet details, whereas the higher resolution preserves intricate temporal variations.}

    \Description{The figure presents five images of a QUIC flow at resolutions of $16 \times 16$, $32 \times 32$, $64 \times 64$, $128 \times 128$, and $256 \times 256$. Each image captures the packet activity within a $0.1$-second window, with increasing detail as resolution increases.}
    \label{fig:different-resolutions}
\end{figure}

\subsection{Dataset Characteristics and Coverage}
\textit{VisQUIC} captures QUIC traffic across multiple implementations, including Google’s Chromium QUIC~\citep{chromiumquiche}, Facebook’s mvfst~\citep{mvfst}, and Cloudflare’s quiche~\citep{quiche}. The dataset spans web traffic from services such as YouTube, Facebook, Discord, and independent news sites, ensuring a diverse sample of real-world QUIC behaviors.
    
To quantify the dataset's scope, Table~\ref{tab:combined-table1} presents the number of traces and generated images for selected web servers. The dataset covers a wide range of services, including social media platforms, content delivery networks, and independent publishers, providing a representative view of QUIC traffic patterns. As shown in Table~\ref{tab:combined-table1}, the number of traces varies significantly across web servers, with Cloudflare contributing the largest volume of traces.


\begin{table}
\caption{Summary statistics of QUIC traces and the number of images per dataset for each web server.}
% \tiny
% \small
\begin{tabular}{|p{2.2cm}|p{1.3cm}|p{0.9cm}|p{1.2cm}|c|}
\hline
\centering \textbf{Web Server} & \centering \textbf{Websites} & \centering \textbf{Traces} & \centering \textbf{$T=0.1$} & \textbf{$T=0.3$} \\ \hline
\centering youtube & \centering 399 & \centering 2,109 & \centering 139,889 & 54,659 \\ \hline
\centering semrush & \centering 1,785 & \centering 9,489 & \centering 474,716 & 221,477 \\ \hline
\centering discord & \centering 527 & \centering 7,271 & \centering 623,823 & 235,248 \\ \hline
\centering instagram & \centering 3 & \centering 207 & \centering 17,003 & 7,112 \\ \hline
\centering mercedes-benz & \centering 46 & \centering 66 & \centering 9,987 & 2,740 \\ \hline
\centering bleacherreport & \centering 1,798 & \centering 8,497 & \centering 781,915 & 331,530 \\ \hline
\centering nicelocal & \centering 1,744 & \centering 1,666 & \centering 148,254 & 48,900 \\ \hline
\centering facebook & \centering 13 & \centering 672 & \centering 25,919 & 10,988 \\ \hline
\centering pcmag & \centering 5,592 & \centering 13,921 & \centering 1,183,717 & 385,797 \\ \hline
\centering logitech & \centering 177 & \centering 728 & \centering 56,792 & 28,580 \\ \hline
\centering google & \centering 1,341 & \centering 2,149 & \centering 81,293 & 29,068 \\ \hline
\centering cdnetworks & \centering 902 & \centering 2,275 & \centering 207,604 & 85,707 \\ \hline
\centering independent & \centering 3,340 & \centering 3,453 & \centering 176,768 & 68,480 \\ \hline
\centering cloudflare & \centering 26,738 & \centering 44,700 & \centering 1,347,766 & 341,488 \\ \hline
\centering jetbrains & \centering 35 & \centering 1,096 & \centering 34,934 & 18,470 \\ \hline
\centering pinterest & \centering 43 & \centering 238 & \centering 6,465 & 2,360 \\ \hline
\centering wiggle & \centering 4 & \centering 0 & \centering 0 & 0 \\ \hline
\centering cnn & \centering 27 & \centering 2,127 & \centering 91,321 & 59,671 \\ \hline
\end{tabular}
\label{tab:combined-table1}
\end{table}

\subsection{Dataset Accessibility and Benchmarking Tools}
To support reproducibility and ease of use, \textit{VisQUIC} is publicly available for academic and research purposes. The dataset, along with documentation, sample traces, and pre-processing scripts, can be accessed through our GitHub repository~\footnote{\url{https://github.com/robshahla/VisQUIC}}.

\textbf{Reproducibility and Docker-Based Environment.}  
To ensure that researchers can easily process and analyze QUIC traffic, we provide a \textbf{containerized processing environment} via Docker. The repository includes a \texttt{Dockerfile} and an executable script, allowing users to set up an analysis pipeline in a standardized environment.

\textbf{Benchmarking Tools.}  
To assist researchers in working with the dataset, the repository also includes:\begin{itemize}
    \item \textbf{Reference implementations} for encrypted traffic classification.
    \item \textbf{Re-processing scripts} for filtering, decrypting, and visualizing QUIC traces.
    \item \textbf{Standardized evaluation} metrics for benchmarking encrypted traffic models.
\end{itemize}

\textbf{Dataset Documentation.}  
Detailed setup instructions, preprocessing guidelines, and dataset structure descriptions can be found in the VisQUIC repository’s README file. 

By combining raw QUIC traces, SSL keys, and optional image-based representations, \textit{VisQUIC} establishes a \textbf{benchmarking standard for encrypted traffic research}, enabling reproducible and scalable experiments in security, networking, and machine learning.

% VisQUIC is a large-scale dataset designed to facilitate benchmarking and research in encrypted traffic analysis. It contains over \textbf{100,000 labeled QUIC traces} collected from \textbf{44,000+ websites} over a four-month period. Unlike existing datasets, VisQUIC provides \textbf{SSL keys} to enable controlled decryption, making it a unique resource for studying encrypted QUIC traffic. Additionally, VisQUIC supports an \textbf{optional image-based representation}, allowing machine learning researchers to explore novel approaches for encrypted traffic analysis.

% \subsection{Dataset Collection and Structure}
% To ensure broad coverage, we collected QUIC traces from two residential networks across different continents, capturing diverse network conditions and geographical variations. Data collection was conducted throughout all the hours of the day, enabling analysis of traffic behavior under varying load conditions.

% \subsection{Dataset Collection and Structure}
% To ensure broad coverage, we collected QUIC traces from two residential networks across different continents, capturing diverse network conditions and geographical variations. Data collection was conducted throughout all hours of the day, enabling analysis of traffic behavior under varying load conditions.

% The dataset was built using active probing of websites that support HTTP/3, selected from the Tranco list~\citep{tranco}, a reliable ranking of the most visited domains. We used \textbf{Headless Chrome}~\citep{headless} in incognito mode with caching disabled to ensure consistency across requests. Each website was requested sequentially, ensuring that every QUIC connection was independent of previous traffic. This methodology eliminates caching effects and session resumption artifacts, allowing for a clean and reproducible dataset.

% To better capture general web traffic, the dataset focuses on traces from sequential web page requests rather than video streaming. The decision to prioritize page requests stems from the limited number of web servers that stream video over QUIC, which restricts server-side traffic diversity. In contrast, web page requests reflect a broader range of application-layer interactions, encompassing various content types, third-party services, and server-side behaviors. Furthermore, video streaming traffic is heavily influenced by adaptive bitrate algorithms and buffering mechanisms controlled by the server, making it less dependent on network conditions. By focusing on web page requests, the dataset provides a more representative view of how QUIC operates across different web services.

% While \textit{VisQUIC} currently emphasizes web page traffic, future work should explore dataset extensions that incorporate varying bandwidth conditions, mobile network scenarios, and additional browsers beyond Chrome. Such extensions would provide a more comprehensive understanding of QUIC traffic across diverse environments.

% \textbf{Traffic Capture and Encryption Data.}  
% QUIC traffic was captured using \textbf{Tshark}~\citep{merino2013instant} in \textbf{packet capture (PCAP)} format, retaining only QUIC packets to focus on encrypted traffic analysis. Each PCAP file is accompanied by its corresponding \textbf{SSL keys}, allowing controlled decryption for research requiring payload inspection.
% \subsection{Optional Image-Based Representation for ML Research}
% In addition to raw network traces, VisQUIC provides an \textbf{optional image-based representation} to support machine learning applications. This approach builds upon prior work on network traffic visualization~\citep{shapira2019flowpic, golubev2022image}, enhancing existing methods by introducing an RGB-based representation that encodes packet arrival times, sizes, and directions. Unlike previous work, which primarily relied on single-channel grayscale representations, our method leverages separate color channels to differentiate between client-to-server and server-to-client traffic. This enhancement preserves crucial directional and temporal relationships, making it particularly effective for analyzing HTTP/3 multiplexing patterns within QUIC traffic.

% Figure~\ref{fig:image-const} illustrates the conversion process:
% \begin{enumerate} 
%     \item \textbf{Extract metadata}: Arrival time, packet size, and direction (client-to-server or server-to-client).
%     \item \textbf{Time and size binning}: Divide the trace into \textit{M} time bins and \textit{N} size bins.
%     \item \textbf{Histogram construction}: Count packets in each bin separately for each direction.
%     \item \textbf{Image creation}: Map histogram values to an RGB image, where red represents server-to-client packets and green represents client-to-server packets.
% \end{enumerate}
% This optional representation allows deep learning models to extract meaningful traffic patterns, even from encrypted traffic. However, VisQUIC remains primarily a raw QUIC trace dataset, with image-based representations serving as an additional resource for machine learning research.
% \begin{figure}[t] 
% \centering \includegraphics[width=1\linewidth]{figforpaper/image-construction.pdf} 
% \caption{Construction of an image from a QUIC trace. (a) Raw packet metadata captures timing, size, and directional information. (b) Packets are binned by time and length, creating histograms for client-to-server (green) and server-to-client (red) traffic. (c) The final RGB representation preserves temporal relationships and directionality, where pixel intensity indicates packet density.}
% \label{fig:image-const} 
% \end{figure}
% \subsection{Dataset Characteristics and Coverage}
% VisQUIC captures QUIC traffic across \textbf{multiple implementations}, including Google’s Chromium QUIC~\citep{chromiumquiche}, Facebook’s mvfst~\citep{mvfst}, and Cloudflare’s quiche~\citep{quiche}. The dataset spans web traffic from services such as YouTube, Facebook, Discord, and independent news sites, ensuring a diverse sample of real-world QUIC behaviors. Table~\ref{tab:combined-table1} summarizes the dataset's scope, listing the number of traces and images collected from each web server.

% \begin{table}
% \caption{Summary statistics of QUIC traces and the number of images per dataset for each web server.}
% % \tiny
% % \small
% \begin{tabular}{|p{2.2cm}|p{1.3cm}|p{0.9cm}|p{1.2cm}|c|}
% \hline
% \centering \textbf{Web Server} & \centering \textbf{Websites} & \centering \textbf{Traces} & \centering \textbf{$T=0.1$} & \textbf{$T=0.3$} \\ \hline
% \centering youtube & \centering 399 & \centering 2,109 & \centering 139,889 & 54,659 \\ \hline
% \centering semrush & \centering 1,785 & \centering 9,489 & \centering 474,716 & 221,477 \\ \hline
% \centering discord & \centering 527 & \centering 7,271 & \centering 623,823 & 235,248 \\ \hline
% \centering instagram & \centering 3 & \centering 207 & \centering 17,003 & 7,112 \\ \hline
% \centering mercedes-benz & \centering 46 & \centering 66 & \centering 9,987 & 2,740 \\ \hline
% \centering bleacherreport & \centering 1,798 & \centering 8,497 & \centering 781,915 & 331,530 \\ \hline
% \centering nicelocal & \centering 1,744 & \centering 1,666 & \centering 148,254 & 48,900 \\ \hline
% \centering facebook & \centering 13 & \centering 672 & \centering 25,919 & 10,988 \\ \hline
% \centering pcmag & \centering 5,592 & \centering 13,921 & \centering 1,183,717 & 385,797 \\ \hline
% \centering logitech & \centering 177 & \centering 728 & \centering 56,792 & 28,580 \\ \hline
% \centering google & \centering 1,341 & \centering 2,149 & \centering 81,293 & 29,068 \\ \hline
% \centering cdnetworks & \centering 902 & \centering 2,275 & \centering 207,604 & 85,707 \\ \hline
% \centering independent & \centering 3,340 & \centering 3,453 & \centering 176,768 & 68,480 \\ \hline
% \centering cloudflare & \centering 26,738 & \centering 44,700 & \centering 1,347,766 & 341,488 \\ \hline
% \centering jetbrains & \centering 35 & \centering 1,096 & \centering 34,934 & 18,470 \\ \hline
% \centering pinterest & \centering 43 & \centering 238 & \centering 6,465 & 2,360 \\ \hline
% \centering wiggle & \centering 4 & \centering 0 & \centering 0 & 0 \\ \hline
% \centering cnn & \centering 27 & \centering 2,127 & \centering 91,321 & 59,671 \\ \hline
% \end{tabular}
% \label{tab:combined-table1}
% \end{table}

% \subsection{Dataset Accessibility and Benchmarking Tools}
% To support reproducibility and ease of use, \textit{VisQUIC} is publicly available for academic and research purposes. The dataset, along with documentation, sample traces, and pre-processing scripts, can be accessed through our GitHub repository: \url{https://github.com/robshahla/VisQUIC}. Researchers can use this repository to explore the dataset structure, retrieve sample QUIC traces, and follow setup instructions.

% \textbf{Reproducibility and Docker-Based Environment.}  
% To ensure that researchers can easily process and analyze QUIC traffic, we provide a \textbf{containerized processing environment} via Docker. The repository includes a \texttt{Dockerfile} and an executable script, allowing users to set up an analysis pipeline in a standardized environment. This setup ensures consistency across different systems and facilitates reproducible benchmarking.

% \textbf{Provided Benchmarking Tools.}  
% To assist researchers in working with the dataset, the repository also includes:
% \begin{itemize}
%     \item \textbf{Reference implementations} for encrypted traffic classification.
%     \item \textbf{Pre-processing scripts} for filtering, decrypting, and visualizing QUIC traces.
%     \item \textbf{Standardized evaluation metrics} for benchmarking encrypted traffic models.
% \end{itemize}

% \textbf{Dataset Samples for Quick Exploration.}  
% To facilitate quick exploration, we provide a subset of anonymized QUIC traces in the dataset repository. These sample traces include PCAP files and corresponding SSL keys, allowing researchers to experiment with QUIC decryption and analysis before accessing the full dataset.

% \textbf{Dataset Documentation.}  
% Detailed setup instructions, preprocessing guidelines, and dataset structure descriptions can be found in the VisQUIC repository’s README file: \url{https://github.com/robshahla/VisQUIC}. We encourage researchers to refer to this documentation for best practices in using the dataset.

% By combining raw QUIC traces, SSL keys, and optional image-based representations, \textit{VisQUIC} establishes a \textbf{benchmarking standard for encrypted traffic research}, enabling reproducible and scalable experiments in security, networking, and machine learning.

==> sections/workflow_uses.tex <==
\subsection{Composition}
Each instance is an image associated with a label of the number of responses within that image. Each image in this dataset is labeled with the number of observed HTTP/3 responses; namely, the number of responses that have started to arrive within every time window. To this end, the HTTP/3 frames are analyzed and HTTP/3 HEADERS frames are identified. Similarly, instead of labeling the images with the number of responses, the number of requests can be used as a label instead.

Tables \ref{tab:combined-table}, \ref{tab:01:images-per-label-per-server} and \ref{tab:03:images-per-label-per-server} contain statistics for all images with a label of 20 or less. The files also contain images with high-class labels, and from the captured traces, additional images and labels can be generated. We publish the whole traces dataset, which contains $100,664$ traces in PCAP format, and outline the traces counts in Table~\ref{tab:combined-table}. The traces were collected from various locations. The label for each image presented in the dataset is the number of responses observed during that time window of the image. Further studies can generate more images and more labels. 

When using the traces or images in the dataset for training purposes, one should check if high-class labels of images are present on specific web servers before splitting the traces into sets of out-of-sample web servers. Some web servers lack images with high class values.
\newpage

\subsection{Collection Process}
The process starts with HTTP/3~\citep{rfc9114} GET requests that are generated to various web servers that support HTTP/3, each hosting multiple websites. Requests are issued for up to $3,176$ different websites per web server. Headless Chrome~\citep{headless} is used in incognito mode with the application cache disabled, and the websites are requested sequentially. The generated network traffic traces are captured using Tshark~\citep{merino2013instant} in packet capture (PCAP) format. These traces include only QUIC packets and cover the duration of the website request. Once we retain the time series captured traces, the image datasets generation process can start for these traces. The SSL keys are stored for each trace in a separate file (and are provided in the dataset). These keys are use to decrypt the relevant QUIC packets.

\subsection{Preprocessing/cleaning/labeling}
Images whose class labels were above 20 responses were not part of the training or evaluation for estimating the number of responses in a QUIC connection, due to their rarity in the data. Besides that, the raw data contains all of the data, unfiltered. Preprocessing was done by filtering out packets that are not QUIC packets. Furthermore, a large number of images were identical, and all of the duplicate images were removed. Before the filtering there was $21,100,925$ images, and after there was $5,040,459$ images. We upload the full dataset including the duplicates. The raw data (captured traces) are saved and will also be available along with the images, upon the paper's acceptance using a link.

\subsection{Maintenance}
Both authors are maintaining the dataset on Github and on relevant links. The dataset can be updated and more labels can be added, for example, requests for each image in addition to responses. Moreover, the dataset can evolve to contain more images using different window lengths. Currently, the dataset contains two window lengths of 0.1 and 0.3 seconds.
Errors may be submitted via the bugtracker on Github. More extensive augmentations may be accepted at the authors' discretion.
